Debiasing Continuous-time Nonlinear Autoregressions

We study how to identify a class of continuous-time nonlinear systems defined by an ordinary differential equation affine in the unknown parameter. We define a notion of asymptotic consistency as $(n, h) \to (\infty, 0)$, and we achieve it using a family of direct methods where the first step is differentiating a noisy time series and the second step is a plug-in linear estimator. The first step, differentiation, is a signal processing adaptation of the nonparametric statistical technique of local polynomial regression. The second step, generalized linear regression, can be consistent using a least squares estimator, but we demonstrate two novel bias corrections that improve the accuracy for finite $h$. These methods significantly broaden the class of continuous-time systems that can be consistently estimated by direct methods.

==> src/independence.tex <==
\section{Designing for independence}
\subsection{Why independence?}
\subsection{Staggered windows}
\subsection{Decorrelation property of orthogonal polynomials}
\label{subsection:orthogonal-independence}
\color{black!20!white}
It is a common assumption in linear systems with process noise that the \(w_i\) are Gaussian but not necessarily white (i.i.d.).
In such a case, we can design the filter so that estimated derivatives of different orders are actually independent.

Modify the inner product \eqref{eq:inner-product} to
\begin{align}
  \left\langle
  f, g
  \right\rangle
   & \leq
  % 
  \expect
  \frac{1}{N}
  \sum_{i, j = 1}^N
  f\del{\frac{i}{N}} g\del{\frac{i}{N}} w_i w_j.
\end{align}


